Multimessenger Analysis Strategy for Core-Collapse Supernova Search: Gravitational Waves and Low-energy Neutrinos

Core-collapse supernovae are fascinating astrophysical objects for multimessenger studies. Gravitational waves (GWs) are expected to play a role in the supernova explosion mechanism, but their modelling is also challenging due to the stochastic nature of the dynamics and the vast possible progenitors, and moreover, the GW detection from these objects is still elusive with the already advanced detectors. Low-energy neutrinos will be emitted enormously during the core-collapse explosion and can help for the gravitational wave counterpart search. In this work we develop a multi-messenger strategy to search for such astrophysical objects by exploiting a global network of both low-energy neutrino and gravitational wave detectors. First, we discuss how to improve the detection potential of the neutrino sub-network by exploiting the temporal behaviour of a neutrino burst from a core-collapse supernova. We show that with the proposed approach neutrino detectors can gain at least $10\%$ of detection efficiency at the distance where their efficiency drops. Then, we combine the information provided by GW and neutrino in a multimessenger strategy. In particular, we obtain an increase of the probability to detect the GW signal from a CCSN at $60$ kpc from zero when using only GW analysis to $\sim 33\%$ with our combined GW-$\nu$ approach. Keywords: multimessenger, supernova, core-collapse, low-energy neutrino, gravitational wave.

==> sections/section02.tex <==
\section{Astrophysical Sources of GW \& LEN\label{sec:sources}}


%Here, in section \ref{sec:sources}, we will discuss several things:

%\begin{enumerate}
    %\item
    %GW-LEN: CCSNe \cite{jankarev}, Failed-SNe\cite{O_Connor_2015}, hadron $\rightarrow$ quark novae
    %\\\\
    
    Sources that can produce a copious of LENs are CCSNe (review can be seen in \cite{jankarev}), failed-supernovae (see more in \cite{O_Connor_2015}), as well as quark novae. All of these sources agree on several parameters: the total energy in neutrinos can be of the order of $10^{53}$ ergs, the surge of neutrinos is of the order of 10 seconds, and the average energy of neutrinos is $O(10)$ MeV. Here, we focus our work on the CCSN search.
    
    \subsection{Gravitational Wave Emission}
    
    GWs are produced by quadrupole mass moment rapidly changing in time\footnote{The general explanation of GW can be seen such as in \cite{maggiore2007gravitational}.}. The signal is characterised by temporal evolution of its amplitude ($h_+$ \& $h_\times$). The (putative) GW bursts from CCSNe are modelled with a very broad classes. Depending on the progenitor scenarios (whether they are nonrotating or highly spinning), the signals may have very different models (see review such as \cite{Ott_2009}).
    
    For the highly spinning progenitors, during core collapse, the stellar core will be spun up of a factor of 1000 comparing with the progenitor core rotation, thanks to the conservation of angular momentum. If the pre-collapse core has a spin period of $\sim$ 1 second, then the proto neutron star, after the collapse, will have a spin period of the order of milliseconds. This rapidly millisecond-spinning compact remnant has a rotational energy of about $10^{52}$ erg. GW signals can be produced thanks to magnetorotational hydrodynamic mechanism \cite{gossan2015,Powell2016}. The GW signal from this mechanism is dominated by bounce and subsequent ringdown of the proto neutron star. Strong centrifugal deformation of inner core, which is related to oblateness, due to rapidly rotating precollapse core, gives a large time-varying quadruple mass moment. The characteristic of GW signal for this rapidly rotating CCSNe will have the peak of the detected strain amplitude ($h_+$ \& $h_\times$) of the order of $\sim10^{-21}-10^{-20}$ at a distance $D\sim10$ kpc. The energy produced in GW, $\epsilon_\mathrm{GW}$ will be of the order of $10^{-10}-10^{-8}M_\odot c^2$. Moreover, the frequency will be narrowband with most emitted power lies on $500-800$ Hz. The timescale for this GW burst will be around $\sim10$ ms. An example $h_+$ evolution of a simulated GW signal from this mechanism can be seen in the top panel of Figure 1 in \cite{Powell2016}.
    
    %An example $h_+$ evolution of a simulated GW signal based on magnetorotational mechanism from a rotating CCSN can be seen in figure \ref{fig:magrot}.
    
    % \begin{figure}[!ht]
    % \centering
    %   \includegraphics[width=.7\linewidth]{figures/magrot.png}
    %   \caption{A plot of $h_+$ evolution from a simulated GWs from a rapidly rotating CCSN based on magnetorotational mechanism, at a distance of 10 kpc. Figure is taken from \cite{Powell2016} based on \cite{dimmelmeier2008}.}
    %   \label{fig:magrot}
    % \end{figure}%
    
    The non-spinning $\nu$-driven CCSNe, which is expected to be more often found, instead, will produce GWs from turbulent convection and Standing Accretion Shock Instability (SASI) \cite{blondin2003}. In this CCSN type, postbounce core is unstable to convection. Immediately, negative entropy gradient behind the stalled shock is formed and the prompt convection carries on, giving rise to a GW burst. Moreover, when the postbounce evolution proceeds, $\nu$-heating sets up negative entropy gradient in the gain layer behind the shock, leading to the \textit{$\nu$-driven convection}. Simultaneously, the $\nu$-diffusion establishes negative lepton gradient in the mantle of proto neutron star, giving rise to \textit{proto neutron star convection}. The frequency content in the neutrino mechanism is robust, but the phase is stochastic (due to turbulence). The signal is long lasting of about $\sim0.3-2$ seconds. The GW strain amplitude is about 1 order of magnitude weaker than from that of the rapidly spinning, $h_+$ (and $h_\times$)$\approx10^{-22}$ at the distance $D=10$ kpc. The energy in gravitational waves $\epsilon_\mathrm{GW}$ is of the order of $\sim10^{-11}-10^{-9}M_\odot c^2$. An example of the $h_+$ evolution from a simulated GW signal from this mechanism is shown in the bottom panel of Figure 1 in \cite{Powell2016}.
    
    %An example of the $h_+$ evolution from a simulated GW signal due to $\nu$-mechanism (convection and SASI) from a CCSN at 10 kpc can be seen in figure \ref{fig:sasi}. This model shows us that the GW signal can last up to $O(1)$ second with strong spikes early on and around 600 milliseconds after the bounce.
    
    
    % \begin{figure}[!ht]
    % \centering
    %   \includegraphics[width=.7\linewidth]{figures/sasi.png}
    %   \caption{A plot of $h_+$ evolution from a simulated GWs from a non-rotating CCSN due to convection and SASI, as seen by an equatorial observer at 10 kpc. Figure is taken from \cite{Powell2016} based on the work of \cite{murphy2009}.}
    %   \label{fig:sasi}
    % \end{figure}%
    
    All in all, we can say that we have several models that are quite broad for this kind of source. Thus, matched-filtering based analysis pipelines that are used to search GWs from blackhole/neutron star binaries\footnote{Matched filter uses a bank of templates from some robust model of a signal and then cross-correlate the templates with the data. This method is popular for the GW searches for binary mergers of compact objects. Notable pipelines are \texttt{PyCBC} \cite{alex_nitz_2020} and \texttt{GstLAL} \cite{chad_hanna2020}.} cannot be optimum for our problem.
    
    
    %This source has a broad possible GW duration depending on the mechanisms producing this collapsing object \cite{Powell2016}. This may range from the order of $\sim10$ms to $2$ seconds \cite{Powell2016}.
    
    In fact, there has been a study on the optically targeted search of this GW signal with Advanced LIGO-Virgo detectors by \texttt{cWB} pipeline \cite{em_gw_ccsne}. The study shows the efficiency of the order of 50\% in the distance of 5 kpc. Taking into account the rate of CCSNe is of the order of 3 events per century in our galaxy ($O(20)$ kpc) itself \cite{Cappellaro2000,diehl2006,maggiore2018}, this is indeed quite a limited distance.
    
    Nevertheless, a multimessenger strategy may expand the detection horizon via coincidence analysis by lowering the background distribution curve and therefore increasing the significance of coincidences. This may give us a new strategy to reevaluate sub-threshold candidates in GW data.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
    
    \subsection{Low-Energy Neutrino Emission}
    \label{subsec:len_emission}
    
    Supernova progenitors already produce strong-luminosity MeV-neutrinos from thermal emission of advanced burning phases, for example the Si burning, even before the collapsing phase. These pre-supernova neutrinos could possibly be detected \cite{ODRZYWOLEK2004303,Kato_2015,Asakura2016,yoshida} by the ultrapure liquid scintillator detectors such as Borexino \cite{borex}, KamLAND \cite{kamland}, JUNO \cite{juno}, as well as DUNE \cite{dune} (or even Super Kamiokande \cite{superK} with the help of Gadolinium). The main detection channel to detect these low-energy CCSN neutrinos is basically the inverse beta decay happening in neutrino detectors,
    \begin{equation}
        \bar{\nu}_e+p\rightarrow n + e^+.
        \label{eq:ibd}
    \end{equation}
    KamLAND collaboration has studied that their detector can detect these pre-supernova neutrinos from a star with a mass of $25M_\odot$ at a distance less than 690 pc with $3\sigma$ significance before the supernova, dependent on the neutrino mass ordering and background levels \cite{Asakura2016}.
    
    During the Fe-core collapse (see \cite{pagliarolitesi,jankarev,Muller2019,Vitagliano2019} for more details in the processes), electron neutrinos are produced by electron captures on heavy nuclei and few free protons. Then, there will be neutrino trapping when the core density is of the order of $10^{12}$ g/cm$^3$. Around the time of trapping $\nu_e$ luminosity reaches $\sim10^{53}$ erg/s with the mean energy of $O(10)$ MeV. The trapping makes a small dip of luminosity due to the fact that neutrinos only come from a narrow region around the newly formed neutrinosphere. Neutrino emission again increases rapidly after the core bounce as newly formed shock propagates into regions of sufficiently low density and reaches neutrinosphere thanks to the shock heating and low optical depth. The dominant production is still $\nu_e$ due to the high $Y_e$ in the shock. The luminosity of this burst of neutrinos can reach $\sim3.5\times10^{53}$ erg/s, known as neutronization burst. A Mton water Cherenkov detector like Hyper Kamiokande \cite{hyperK} can observe this burst, which would be a standard candle with distance error measurement of $\sim5\%$. Moreover, the nonobservation of this peak will support the normal mass hierarchy in neutrinos, while the observation will be consistent with the inverted hierarchy (see more in \cite{kachelriess2005}).
    
    Around ten of millisecond timescale after the bounce, the CCSN develops an accretion shock lying on $\sim100-200$ km from the center. Neutrino emission for electron and heavy flavor is quite different in this phase. For all flavors during this phase, there is a diffusive flux to proto neutron star surface region driven by temperature gradient and neutrino chemical potential. For electron flavor neutrinos, the emission is not only due to the diffusion of thermal energy from the proto neutron star core, but also from the accretion. During accretion phase, $10-20\%$ of $\nu_e-\bar{\nu}_e$ energy is converted to thermal energy and can revive the shock. The timescale in this phase is $t\sim0.5$ sec. Simulations show that the mean energy of electron antineutrinos $\langle E_{\bar{\nu}_e}\rangle$ is somewhat proportional to proto neutron star mass during the accretion.
    
    During the cooling phase, the electron flavor and heavy flavor luminosity become relatively similar. The luminosity of all flavors decreases roughly exponentially with a decay time-scale of seconds. Then, a fraction of infalling materials adds to the proto neutron star until the explosion. The proto neutron star evolves to be a neutron star. Most of CCSN energy is emitted in this phase (called cooling phase), accounting for $\sim90\%$ in the form of all neutrino and antineutrino species with high luminosity. The primary production of neutrinos in this phase is the neutral current (for all neutrino and antineutrino species).
    
%     =========
    
    
    
%     %\item LEN from CCSNe,
%      %   \begin{itemize}
%             %\item
%             SN1987A detection\cite{hirata1987,Bionta1987,alexeyev}
%             %\item
%             cite some models; energy in neutrino, duration, etc
%             %\item
%             Pagliaroli parametrization\cite{pagliaroli2009}
%             %\item
%             current detector status
%             %\item
%             how to detect: LVD analysis paper\cite{Agafonova2014}, SK offline\cite{Ikeda2007} + online\cite{Abe2016}, Icecube\cite{icecube} ???
%             %\item
%             SNEWS\cite{Antonioli2004};
%             %\item
%             pre-SN neutrinos: KamLAND\cite{Asakura2016}
%             %\item
%             rate and distribution \cite{maggiore2018}
%             %\item
%             triangulation from Kate paper\cite{triangul_kate}
%             %\item
%             Gadolinium for SK
%             %\item
%             Failed-SN from Evan O'Connor
%             %\item
%             Claudio's paper (xi)\cite{Casentini2018}
%             %\item
%             Expanding core collapse horizon\cite{halim2019},
%             \begin{equation}
%             f^\mathrm{im}_i=N\times \sum_{k=m_i}^\infty P(k),
%             \label{eq:fim_prob}
%             \end{equation}
%             where,
%             \begin{equation}
%             P(k)=\frac{(f_\mathrm{bkg}w)^k e^{-f_\mathrm{bkg}w}}{k!}.
%             \label{eq:poiss_pdf}
%             \end{equation}
%             Then, becomes,
%             \begin{equation}
%             \begin{split}
%             F^\mathrm{im}_i = & 8640\times  \sum_{k=m_i}^\infty  P(k,\xi) \\
%             = & 8640 \times \sum_{k=m_i}^\infty  P(\xi | k)P(k) \\
%             = & 8640 \times \sum_{k=m_i}^\infty P(k) \int_{\xi=\xi_i}^\infty PDF(\xi\geq\xi_i|k) d\xi.
%             \end{split}
%             \label{eq:newfim_1}
%             \end{equation}
%             The proof can be seen in appendix \ref{}


%         %\end{itemize}
%     %\item
%     GW models, energy, progenitors, signals
%         \begin{itemize}
%             \item Analysis: Marco's paper on ML, cWB\cite{Klimenko_2004,Klimenko2008,dragotesi,Necula_2012,cWB_caltech}
%             \item EM triggered paper: rate and efficiency\cite{em_gw_ccsne}
%             \item Gossan paper: injections, efficiency\cite{gossan2015}
%         \end{itemize}
%     %\item
%     Time delay of GW \& LEN
% %\end{enumerate}























%\section{Math and Equations}

% Inline math may be typeset using the \verb+$+ delimiters. Bold math
% symbols may be achieved using the \verb+bm+ package and the
% \verb+\bm{#1}+ command it supplies. For instance, a bold $\alpha$ can
% be typeset as \verb+$\bm{\alpha}$+ giving $\bm{\alpha}$. Fraktur and
% Blackboard (or open face or double struck) characters should be
% typeset using the \verb+\mathfrak{#1}+ and \verb+\mathbb{#1}+ commands
% respectively. Both are supplied by the \texttt{amssymb} package. For
% example, \verb+$\mathbb{R}$+ gives $\mathbb{R}$ and
% \verb+$\mathfrak{G}$+ gives $\mathfrak{G}$

% In \LaTeX\ there are many different ways to display equations, and a
% few preferred ways are noted below. Displayed math will center by
% default. Use the class option \verb+fleqn+ to flush equations left.

% Below we have numbered single-line equations; this is the most common
% type of equation in \textit{Physical Review}:
% \begin{eqnarray}
% \chi_+(p)\alt{\bf [}2|{\bf p}|(|{\bf p}|+p_z){\bf ]}^{-1/2}
% \left(
% \begin{array}{c}
% |{\bf p}|+p_z\\
% px+ip_y
% \end{array}\right)\;,
% \\
% \left\{%
%  \openone234567890abc123\alpha\beta\gamma\delta1234556\alpha\beta
%  \frac{1\sum^{a}_{b}}{A^2}%
% \right\}%
% \label{eq:one}.
% \end{eqnarray}
% Note the open one in Eq.~(\ref{eq:one}).

% Not all numbered equations will fit within a narrow column this
% way. The equation number will move down automatically if it cannot fit
% on the same line with a one-line equation:
% \begin{equation}
% \left\{
%  ab12345678abc123456abcdef\alpha\beta\gamma\delta1234556\alpha\beta
%  \frac{1\sum^{a}_{b}}{A^2}%
% \right\}.
% \end{equation}

% When the \verb+\label{#1}+ command is used [cf. input for
% Eq.~(\ref{eq:one})], the equation can be referred to in text without
% knowing the equation number that \TeX\ will assign to it. Just
% use \verb+\ref{#1}+, where \verb+#1+ is the same name that used in
% the \verb+\label{#1}+ command.

% Unnumbered single-line equations can be typeset
% using the \verb+\[+, \verb+\]+ format:
% \[g^+g^+ \rightarrow g^+g^+g^+g^+ \dots ~,~~q^+q^+\rightarrow
% q^+g^+g^+ \dots ~. \]


% \subsection{Multiline equations}

% Multiline equations are obtained by using the \verb+eqnarray+
% environment.  Use the \verb+\nonumber+ command at the end of each line
% to avoid assigning a number:
% \begin{eqnarray}
% {\cal M}=&&ig_Z^2(4E_1E_2)^{1/2}(l_i^2)^{-1}
% \delta_{\sigma_1,-\sigma_2}
% (g_{\sigma_2}^e)^2\chi_{-\sigma_2}(p_2)\nonumber\\
% &&\times
% [\epsilon_jl_i\epsilon_i]_{\sigma_1}\chi_{\sigma_1}(p_1),
% \end{eqnarray}
% \begin{eqnarray}
% \sum \vert M^{\text{viol}}_g \vert ^2&=&g^{2n-4}_S(Q^2)~N^{n-2}
%         (N^2-1)\nonumber \\
%  & &\times \left( \sum_{i<j}\right)
%   \sum_{\text{perm}}
%  \frac{1}{S_{12}}
%  \frac{1}{S_{12}}
%  \sum_\tau c^f_\tau~.
% \end{eqnarray}
% \textbf{Note:} Do not use \verb+\label{#1}+ on a line of a multiline
% equation if \verb+\nonumber+ is also used on that line. Incorrect
% cross-referencing will result. Notice the use \verb+\text{#1}+ for
% using a Roman font within a math environment.

% To set a multiline equation without \emph{any} equation
% numbers, use the \verb+\begin{eqnarray*}+,
% \verb+\end{eqnarray*}+ format:
% \begin{eqnarray*}
% \sum \vert M^{\text{viol}}_g \vert ^2&=&g^{2n-4}_S(Q^2)~N^{n-2}
%         (N^2-1)\\
%  & &\times \left( \sum_{i<j}\right)
%  \left(
%   \sum_{\text{perm}}\frac{1}{S_{12}S_{23}S_{n1}}
%  \right)
%  \frac{1}{S_{12}}~.
% \end{eqnarray*}

% To obtain numbers not normally produced by the automatic numbering,
% use the \verb+\tag{#1}+ command, where \verb+#1+ is the desired
% equation number. For example, to get an equation number of
% (\ref{eq:mynum}),
% \begin{equation}
% g^+g^+ \rightarrow g^+g^+g^+g^+ \dots ~,~~q^+q^+\rightarrow
% q^+g^+g^+ \dots ~. \tag{2.6$'$}\label{eq:mynum}
% \end{equation}

% \paragraph{A few notes on \texttt{tag}s} 
% \verb+\tag{#1}+ requires the \texttt{amsmath} package. 
% Place the \verb+\tag{#1}+ command before the \verb+\label{#1}+, if any. 
% The numbering produced by \verb+\tag{#1}+ \textit{does not affect} 
% the automatic numbering in REV\TeX; 
% therefore, the number must be known ahead of time, 
% and it must be manually adjusted if other equations are added. 
% \verb+\tag{#1}+ works with both single-line and multiline equations. 
% \verb+\tag{#1}+ should only be used in exceptional cases---%
% do not use it to number many equations in your paper. 
% Please note that this feature of the \texttt{amsmath} package
% is \emph{not} compatible with the \texttt{hyperref} (6.77u) package.

% Enclosing display math within
% \verb+\begin{subequations}+ and \verb+\end{subequations}+ will produce
% a set of equations that are labeled with letters, as shown in
% Eqs.~(\ref{subeq:1}) and (\ref{subeq:2}) below.
% You may include any number of single-line and multiline equations,
% although it is probably not a good idea to follow one display math
% directly after another.
% \begin{subequations}
% \label{eq:whole}
% \begin{eqnarray}
% {\cal M}=&&ig_Z^2(4E_1E_2)^{1/2}(l_i^2)^{-1}
% (g_{\sigma_2}^e)^2\chi_{-\sigma_2}(p_2)\nonumber\\
% &&\times
% [\epsilon_i]_{\sigma_1}\chi_{\sigma_1}(p_1).\label{subeq:2}
% \end{eqnarray}
% \begin{equation}
% \left\{
%  abc123456abcdef\alpha\beta\gamma\delta1234556\alpha\beta
%  \frac{1\sum^{a}_{b}}{A^2}
% \right\},\label{subeq:1}
% \end{equation}
% \end{subequations}
% Giving a \verb+\label{#1}+ command directly after the \verb+\begin{subequations}+, 
% allows you to reference all the equations in the \texttt{subequations} environment. 
% For example, the equations in the preceding subequations environment were
% Eqs.~(\ref{eq:whole}).

% \subsubsection{Wide equations}
% The equation that follows is set in a wide format, i.e., it spans the full page. 
% The wide format is reserved for long equations
% that cannot easily be set in a single column:
% \begin{widetext}
% \begin{equation}
% {\cal R}^{(\text{d})}=
%  g_{\sigma_2}^e
%  \left(
%   \frac{[\Gamma^Z(3,21)]_{\sigma_1}}{Q_{12}^2-M_W^2}
%   +\frac{[\Gamma^Z(13,2)]_{\sigma_1}}{Q_{13}^2-M_W^2}
%  \right)
%  + x_WQ_e
%  \left(
%   \frac{[\Gamma^\gamma(3,21)]_{\sigma_1}}{Q_{12}^2-M_W^2}
%   +\frac{[\Gamma^\gamma(13,2)]_{\sigma_1}}{Q_{13}^2-M_W^2}
%  \right)\;. 
%  \label{eq:wideeq}
% \end{equation}
% \end{widetext}
% This is typed to show how the output appears in wide format.
% (Incidentally, since there is no blank line between the \texttt{equation} environment above 
% and the start of this paragraph, this paragraph is not indented.)


==> sections/section05.tex <==
 \section{Joint GW-LEN Analysis\label{sec:multi}}
 
 Diagram explanation
 
 \begin{enumerate}
     \item[A] Coincidence time window: time of lum curve of neutrino from CCSNe
     \item[B] Joint GW+LEN signif!
     \item[C] BG trigger generation
     \item[D] Individual detection
     \item[E] Statistical detection of multiple sources: collective method
     \item[F] Simul of Astrophy signals: to check sensitivity of the algorithm; monte carlo
     \item[G] Population estimation
     \item[H] Estimated sensitivity: What about the final result as a \textit{proof-of-concept}????
 \end{enumerate}
